Introducing the Plaid Model

We introduce and prove some basic results about a combinatorial model which produces embedded polygons in the plane. The model is closely related to outer billiards on kites, and also is related to corner percolation, to Hooper's Truchet tile system, to self-similar tilings, and to polyhedron exchange transformations.

==> 4tiles.tex <==

\section{The PET Equivalence Theorem}

\subsection{Oriented Version}
\label{orient}

In this chapter we deduce the PET Equivalence
Theorem from the Isomorphism Theorem.
This is mainly just a matter of
interpretation.

The tile description 
allows for the possibility of orienting
the loops in the model.  There are $12+1$
ways of drawing a directed edge in a square
tile which connects up the midpoints of
different sides.  Aside from the empty
tile, the remaining $12$ tiles are indexed
by ordered $2$-element subsets of
$\{N,S,E,W\}$.   As a first step
in proving the PET Isomorphism Theorem,
we explain the oriented version of
our model.

We partition $[0,1] \times \R^3$ by
thinking of this space as the universal
cover of $X$ and then lifting the pieces of
the partition.  We then quotient out by
the index $2$ affine subgroup $\Lambda'$ which,
for each parameter $P$, acts as the lattice
generated by
\begin{equation}
(4,2P,2P), \hskip 30 pt
(0,2,0), \hskip 30 pt (0,0,2).
\end{equation}
We let $\widehat X$ denote this quotient.
We think of 
$$[0,1] \times [-2,2] \times [-1,1]^2$$
as the fundamental domain for $\widehat X$.
This turns out to be the most symmetric
choice.  We can identify $X$ with the
middle half of this fundamental domain,
namely
$$[0,1] \times [-1,1] \times [-1,1]^2,$$

We enhance the labels on $\widehat X$
in the following way:
\begin{itemize}
\item For $T \in [-1,1]$ we use the labels as they
are ordered in Figure 3.1.
\item For $T \in [-2,-1] \cup [1,2]$ we use the labels 
in the reverse order.  So, for instance, the piece
labeled NW in Figure 3.1 would be labeled WN in
the other half of $\widehat X$.
\end{itemize}

In the next section we will give an unsatisfying
computational proof that our enhanced classifying
space produces coherent tilings.  After doing
this, we will interpret the result in terms
of polyhedron exhange transformations.
The interested reader can see the oriented version
in action on my computer program.

\subsection{Proof of Coherent Orientations}

We would like to see, for each parameter $p/q$, that the
classifying pair $(\widehat \Xi_P,\widehat X_P)$,
with $P=2p/(p+q)$, produces
a coherently oriented tiling in the following sense: If two connectors
in adjacent tiles both involve the common edge, then
one connector points into the edge and the other points
out of it.  Since we have a double cover of the
original classifying pair, the Isomorphism Theorem
tells that we only have to worry about the orientations,
and not the actual matching of the connectors.

We will explain the
argument in one of $8$ cases.  The argument works
the same in all cases.  Define
\begin{equation}
\widehat X_{S \downarrow}=\widehat X_{ES} \cup \widehat X_{WS} \cup
\widehat X_{NS}
\end{equation}
as the union of all regions in $\widehat X$ which assign
tiles that point into their south edge.  This set
is a finite union of $4$ dimensional convex integral polytopes.
In a similar way, define
$\widehat X_{N,\downarrow}$ as the set of all regions which
assign tiles that point out of their north edges.

There is an integral affine transformation
$\Upsilon: \widehat X \to \widehat X$ which has the property that
\begin{equation}
\Upsilon \circ \Xi(x,y)=\Xi(x,y-1).
\end{equation}
From Equation \ref{map}, we get
\begin{equation}
\Upsilon(P,\widehat T,U_1,U_2)=(P,\widehat T-2,U_1,U_2-2P) \hskip 10 pt
{\rm mod\/} \hskip 10 pt \Lambda.
\end{equation}
This map is a fiberwise translation.
In particular, the image of a finite union of $K$ convex integer
polytopes under $\Upsilon$ is again a finite union of $K$
convex integer polytopes.  

The statement that every tile which points into the south edge
meets a tile below it that points out of the north edge is
equivalent to the statement that
\begin{equation}
\label{mesh}
\Upsilon(\widehat X_{S,\downarrow})=\widehat X_{N,\downarrow}.
\end{equation}

Recall from the description in \S \ref{partition0}
that $X$ is partitioned into $3$ zones.
So, $\widehat X$ is partitioned into $6$ zones.
More precisely, $\widehat X$ is a fiber bundle
over a union of $6$ integer triangles, and
each zone is the preimage of one of the triangles.
Each of our sets intersects a zone in a
convex integer polytope.  Hence $K=6$.

Say that a {\it triad\/} is a triple of
parameters $\{(P_i,T_i)\}$ for $i=1,2,3$ which
lies in the interior of one of the $6$ triangles
in the base space.

\begin{lemma}
Suppose that Equation \ref{mesh} holds in
the fibers associated to $6$ triads,
one per zone.  Then Equation \ref{mesh}
holds everywhere.
\end{lemma}

\startproof
The two sets in Equation \ref{mesh} intersect
each zone in a convex integer polytope.
Let $L$ and $R$ respectively be the intersection
of the left and right hand sides of
Equation \ref{mesh} with one of the zones.
As we discussed in \S \ref{partition0}, both
$L$ and $R$ are intersect
each interior fiber in a rectangle.
(We mean a fiber over an interior point of the base.)
From this description, 
we have $L=R$ provided that $L$ and $R$ intersect
a triad of fibers in the same way.
\endproof

\begin{lemma}
Suppose that the classifying pair
$(\widehat \Xi_P,\widehat X)$ produces
a coherently oriented tiling
at the parameters $p/q=3/8$ and
$p=4/11$ (corresponding to $P=6/11$ and
$P=8/15$).  Then Equation \ref{mesh}
holds everywhere.
\end{lemma}

\startproof
First we consider some general parameter $p/q$.
Let $\omega=p+q$.  Let $P=2p/\omega$.
Let $\cal C$ denote the set of centers of
the square tiles.
Over any fiber $F$ which contains points
of $\Xi_P({\cal C\/})$, we divide
$F$ into $\omega^2$ squares of side-length
$2/\omega$.  As we discussed in
\S \ref{defined}, the image of
$\Xi_P({\cal C\/}) \cap F$ is exactly
the set of centers of these little squares.

At the same time, 
$\widehat X_{N,\downarrow}$ intersects $F$
in the segments extending the edges of the
little squares.    But the translation
$\Upsilon$ preserves the division of
$\widehat X$ into cubes of side length
$2/\omega$.  Hence $\Upsilon(\widehat X_{S,\downarrow})$
also intersects $F$ in the segments extending the
sides of the little squares.

It follows from Lemma \ref{bijection} that
$\Xi({\cal C\/}) \cap F$ contains every
little square center.  Hence, of our two
sets disagreed in $F$, there would be some
mismatch of orientations we could see in
the tiling.  Since the tiling is coherently
oriented, there is no mismatch.

The parameters $3/8$ and $4/11$ are large
enough so that the image
$$\Xi_{6/11}({\cal C\/}) \cup
\Xi_{8/15}({\cal C\/})$$
contains a triad in every zone.
\endproof


Now we simply inspect the picture for these
two parameters and see that the tiling
produced is coherent.  The parameters involved
are so small that there is no round-off
error in the calculation.


\subsection{Polytope Exchange Transformations}

The data for a polytope exchange transformation is
two partitions of a polytope $Y$ into smaller
polytopes.
\begin{equation}
Y=\bigcup_{i=1}^N L_i=\bigcup_{i=1}^N R_i.
\end{equation}
By {\it partition\/} we mean that the 
smaller pieces have pairwise disjoint interiors.

We insist that there is some translation
$f_i$ so that $f_i(L_i)=R_i$ for all $i$.
These maps piece together to give an almost-everywhere
defined map $F: Y \to Y$.  One defines
$F(p)=f_i(p)$ provided that $p$ lies in the interior
of $L_i$.  The inverse map is defined to be
$F^{-1}(q)=f_i^{-1}(q)$ provided that $q$ lies
in the interior of $R_i$.

A variant of this is to consider $Y$ to
be a flat manifold.  This case really isn't
that different from the polytope case, and indeed
by refining the partitions we can
readily convert between one to the other.
One encounters this situation when one considers
a circle rotation to be a $2$-interval IET.
A refinement of the partition introduces new
points where the map is not, strictly speaking,
defined. However, we will see that this
situation has no impact on our main goals.
In the irrational case, we will study orbits
which are well-defined in either set-up.

For each parameter $p/q$, we set $P=2p/(p+q)$, 
and our space 
is $\widehat X_P$.
The partition is given by
\begin{equation}
\widehat X_{S \downarrow} \cup
\widehat X_{W \leftarrow} \cup
\widehat X_{N \uparrow} \cup
\widehat X_{E \rightarrow}.
\cup \widehat X_0.
\end{equation}
The remaining set $\widehat X_0$ is just the complement.
These sets have an obvious meaning.  We already defined
$\widehat X_{S \downarrow}$.  The set
$\widehat X_{E,\rightarrow}$ is the union of
regions which assign tiles which point into their east edges.
And so on.
The second partition of $\widehat X$ is obtained by
reversing all the arrows.

In other words, the pieces in the first partition
are understood as the ones which specify tiles according
to the edges they point into and the pieces in the
second partition are understood as the ones which specify
tiles according to the edges they point out of.  Both
partitions share the regions which assign the empty tile.

We have $5$ {\it curve following maps\/}.
\begin{itemize}
\item $\Upsilon_0: \widehat X_0 \to \widehat X_0$.
\item $\Upsilon_S: \widehat X_{S \downarrow} \to \widehat X_{N\downarrow}$.
\item $\Upsilon_W: \widehat X_{W \leftarrow} \to \widehat X_{E\leftarrow}$.
\item $\Upsilon_N: \widehat X_{N \uparrow} \to \widehat X_{W\uparrow}$.
\item $\Upsilon_E: \widehat X_{E \rightarrow} \to \widehat X_{W\rightarrow}$.
\end{itemize}
These maps are all translations on their domain.
The map $\Upsilon_0$ is the identity map.  We
considered $\Upsilon_S$ above.  The other maps are
similar.

There is a natural map on $\cal C$, the set of centers
of the square tiles.  We simply follow the directed edge
of the tile centered at $c$
and arrive at the next tile center.  By construction,
 $\widehat \Xi_P$ conjugates this map on
$\cal C$ to our polyhedron exchange transformation.
If we work within the fundamental domain, then
$\widehat \Xi_P$ is a bijection, by Lemma \ref{bijection}.
By construction $\widehat \Xi_P$ sets up a tautological
bijection between the plaid polygons and the
set of orbits of points of the form
$\widehat \Xi(c)$, where $c \in \cal C$.  We call
these orbits {\it special orbits\/}.

By construction $\widehat \Xi_P$
sets up a dynamics-respecting bijection 
the special orbits and the plaid polygons
contained in the fundamental domain, with
respect to the parameter $p/q$.

To get the vector dynamics mentioned in the
PET Equivalence Theorem, we assign the vectors
$(0,-1)$ to the region $\widehat X_{S\downarrow}$, 
and $(-1,0)$ to $\widehat X_{W\leftarrow}$, etc.
When we follow the orbit of
$\Xi(c)$, we get record the list of vectors labeling
the regions successively visited by the point. This gives
vectors $v_1,v_2,v_3$.  We then
accumulate these vectors:
\begin{equation}
c_k=c+\sum_{i=1}^k v_i.
\end{equation}
The vertices $c_0,c_1,c_2,...$ are then the vertices
of the plaid polygon containing $c$.
This is what we mean by saying that the plaid polygons
describe the vector dynamics of the special orbits
of the PET.  This proves the first statement
of the PET Equivalence Theorem.

\subsection{The Global Picture}

We can define an {\it affine polytope exchange\/}
transformation just as above, except that the
maps $f_i$ are affine transformations
rather than translations.  We say that such
dynamical system is {\it fibered\/} if it
is a fiber bundle over some base space such
that the maps preserve each fiber and act
as ordinary PETs there.  

So far, we have been working fiber by fiber.  But the
total space $\widehat X$ is naturally a flat affine
manifold, as we discussed (for the two-fold
quotient) in the previous chapter.
The partitions defined in the previous section piece
together to give a partition of $\widehat X$ into
finitely many convex polytopes.  The polyhedron
exchange maps piece together to give piecewise
affine maps of $\widehat X$.  The definitions
make sense even for irrational parameters.
Thus $\widehat X$ is a fibered piecewise affine
polytope exchange transformation, and the fiber
over $P$ is $\widehat X_P$.

We have
\begin{equation}
\widehat X=([0,1] \times \R^3)/\widehat \Lambda,
\end{equation}
where $\widehat \Lambda$ is a group of
{\it integral\/} affine transformations.
We say that a convex polytope in $\widehat X$ is
{\it integral\/} if one of its lifts to
the universal cover has integer vertices.
Given the nature of our quotient, this definition
is independent of lift.  

The polytopes in both partitions are unions of
finitely many convex polytopes of the kind which
partition the $2$-fold quotient space
$X$.  Thus, the partitions of $\widehat X$
consist of convex integral polytopes.  In
short, $\widehat X$ is a fibered, integral,
piecewise affine polytope exchange transformation.
This proves the second statement of the
PET Equivalence Theorem.

\newpage


==> 5unbound.tex <==
\section{Unbounded Orbits}

\subsection{Taking Limits Carefully}

Let $\{p_k/q_k\}$ be
such that $p_k/q_k \to A$.  Let
$P_k=2p_k/(\omega_k)$ and
let $P=\lim P_k$. 
We have
\begin{equation}
P=\frac{2A}{1+A}.
\end{equation}

Let $\Xi_k$ denote the classifying map
associated to the parameter $p_k/q_k$.
Here $\Xi_k$ maps $\cal C$ into the
space $X_{P_k}$.  
Suppose we have
an auxiliary sequence $Z=\{z_k\}$ of points such that
$z_k \in \Gamma_k$.  We define
\begin{equation}
\Xi^Z_k(c)=\Xi_k(c-z_k).
\end{equation}
We can pass to a subsequence so that the
maps $\{\Xi_k^Z\}$ converge to a
limiting map $\Xi^Z: {\cal C\/} \to X_P$.
We call $Z$ is {\it good seqience\/} if
\begin{equation}
\Xi^Z(0,0)=(\zeta_0,\zeta_1,\zeta_2),
\end{equation}
$\zeta_0$ lies in the group $\Q[P]$ but
$\zeta_1$ and $\zeta_2$ 
do not.  Here $\Q[P]$ is the set of
combinations $r_1+r_2 P$ with $r_1,r_2 \in \Q$.
Recall that $\cal C$ is the set of tile centers.

\begin{lemma}
If $Z$ is a good sequence, then 
$\Xi^Z({\cal C\/})$ is disjoint from
the singular set of the partition of $X_P$.
\end{lemma}

\startproof
For any $c \in \cal C$, the
coordinates of
$\Xi^Z(c)-\Xi^Z(0)$ all lie in $\Q[P]$.
Hence
$\Xi^Z(c)$ lies in a fiber over a point of $\Q[P]$ 
and the other two coordinates do not belong
to $\Q[P]$.  Since our partition consists
of integral polytopes sliced by fibers,
the intersection of our partition walls with
a fiber over $\Q[P]$ consists of horizontal
and vertical lines defined over $\Q[P]$.
Hence, $\Xi^Z(c)$ does not lie in this set.
\endproof

If $\Xi^Z(\cal C)$ is disjoint from the
singular set in $X$, then the lifted
set $\widehat \Xi^Z(\cal C)$ is disjoint
from the singular set in the space
$\widehat X_P$.  Hence, every point
of $\widehat \Xi^Z(\cal C)$ has a
well defined orbit.  By construction,
the polygonal path through
$(0,0)$ is unbounded, because
it is the limit (on a subsequence) of
increasingly long polygons.  Hence
$\widehat \Xi^Z(0,0)$ has an infinite
orbit in the PET defined on $\widehat X_P$
at the parameter $P$.

At least one of the coordinate
projections of our infinite
polygonal path will 
be infinite.  However, we will need to take
some additional care to arrange that both
coordinate projections are infinite.  In
any case, our strategy is to find a good 
sequence $Z=\{z_k\}$.

\subsection{Finding the Good Sequence}

Let $\Gamma_k$ denote the first polygon
associated to $p_k/q_k$.  Let
$y_{k0}$ and $y_{k1}$ be such that
$(0,y_{k0})$ and $(0,y_{k1})$ are the
two points of mass $1$ inside the first block.
These points come within $1$ unit of
$\Gamma_k$.   Indeed, one of the points
$(1/2,y_{kj})$ is the point we called
$z_1$ in the proof of Theorem \ref{first}.








\end{document}








==> Extra/rescale.tex <==




This section is mostly speculative.
We continue with the notation from
Theorem \ref{bigg2}.
Suppose we fix some $\epsilon>0$ and we
consider a sequence $\{\Pi_k\}$ of plaid
polygons with $\Pi_k \subset B_k$
so that 
\begin{equation}
{\rm diameter\/}(\Pi_k)>\epsilon \omega_k.
\end{equation}
Theorem \ref{bigg2} guarantees that
such polygons exist in abundance
once $\epsilon$ is sufficiently small.

For simplicity, we first
first consider the case when $B_k$ is always
the first block.  In this case, the
rescaled sets $\{T_k(\Gamma_{k,M})\}$ and
$\{T_k(\Omega_{k,M})\}$ converge
to $\Gamma_M$ and $\Omega_M$ without
the introduction of an offset $\xi$.
In other words, we get convergence without
taking a subsequence.   We are
interested in understanding the possible
Hausdorff limits of the sequence
$\{T_k(\Pi_k)\}$.  If this sequence
converges, it means that the various
polygons $\Pi_k$ have asymptotically
the same shape, mod scaling.
\newline
\newline
{\bf Coherent Rectangles:\/}
Let $\Gamma=\bigcup \Gamma_M$ and
let $\Omega=\bigcup \Omega_M$.
In both cases, we have a dense set of lines.
We say that a
$\Gamma$-{\it rectangle\/} is a
rectangle whose sides belong to 
$\Gamma$.  Let $R$ be such a
rectangle.  We call $R$
{\it coherent\/} if $\partial R$
contain no light points or if
$\partial R$ contains exactly
$2$ light points, each one
on the interior of a different
edge of $R$.
Notice that this is exactly
the condition used in the Fundamental
Theorem.
\newline
\newline
{\bf Coherent Partitions:\/}
We say that a {\it coherent partition\/} is
a partition of $[0,1]^2$ into
coherent $\Gamma$ rectangles.
My computer program produces coherent
tilings by a recursive subdivision
algorithm.  I start with the grid
$\Gamma_M$ for some $M$.  If there
is some rectangle that is not coherent,
I subdivide that rectangle into two
halves using the line of $\Gamma_{M'}$
for the smallest possible $M'>M$. 
The algorithm alternates between
horizontal and vertical edges,
so that the rectangles stay roughly square.
If the algorithm halts, it produces a
coherent tiling.
In practice, the algorithm works very well.

\begin{conjecture}
The recursive subdivision algorithm
always halts, starting with any
irrational parameter and any
initial choice of $M$.
\end{conjecture}


The conjecture only concerns the case when
$\Omega$ has no offset.  If we add an
offset to $\Omega$, I don't have much
understanding of what happens. Thanks
to the phenomenon of crossing particles,
one can certainly choose offsets which
will defeat the algorithm.
\newline
\newline
{\bf The Associated Tiling and Loops:\/}
Assume that we have a coherent partition.
For each rectangle in the partition,
we can draw a connecting edge which
joins the two light points. The
construction is very similar to what
we did in the previous chapter, except
that we did not use the light points
themselves but rather the centers of
the unit segments containing.  Since
our rectangles might not meet edge-to-edge,
it is better to use the light points
themselves.  When we have added
all these rectangular tiles, all
the light points lie on finitely 
many polygons.  We call these
polygons the {\it loops\/}
associated to the coherent partition.
\newline
\newline
{\bf Approximate Convergence:\/}
Let's again consider our sequence
$\{\Pi_k\}$ of plaid polygons.
Assume that we have a coherent partition
$\Upsilon$
whose largest rectangle has diameter
somewhat smaller than $\epsilon$.
Let $\Upsilon_k$ denote the corresponding
rectangle partition in $[0,\omega_k]^2$.
Once $k$ is sufficiently large,
$\Upsilon_k$ will also be coherent,
and $\Pi_k$ will intersect $\Upsilon_k$
in the same combinatorial pattern
that one of the loops intersects
$\Upsilon$.  Therefore, any
Hausdorff subsequential
limit of the rescaled sequence
$\{T_k(\Pi_k)\}$ will agree with one
of the loops up to an error
of at most $\epsilon$.

At least for the cases shown in Figures
1.1 and 1.2, this kind of structure
explains the coarse similarity between
the two pictures.  Both parameters
are nearly equal, and
$$\tau(4/17)=8/21, \hskip 30 pt
\tau(17/72)=34/89.$$
So $4/17 \approx 17/72$
and $\tau(4/17) \approx \tau(17/72)$.
\newline
\newline
{\bf The Even Expansion:\/}
One natural way to produce tuned sequences
is to start with a quadratic irrational parameter
$A$ and consider what I call the {\it even expansion\/}
of $A$.  This is an infinite sequence
$\{p_k/q_k\}$ which converges to $A$ and has the
property that $|p_{k+1}q_k-p_kq_{k+1}|=1$.
That is, the rationals are joined by edges of
the famous Farey graph.
The sequence $\{p_k/q_k\}$ might not be tuned.
However, it seems to always split into finitely
many subsequences which are irrationally
tuned.  The number of such subsequence is
certainly related to the continued
fraction expansion of $A$, but it has more
to do with how $A$ relates to the level $2$
congruence subgroup $\Gamma_2 \subset PSL_2(\Z)$.
I hope to explore all this in a sequel paper.

For example, if one takes $A=\sqrt 5-2$, then the
even expansion of $A$ is given by
$$\frac{1}{4}, \hskip 20 pt
\frac{4}{17}, \hskip 20 pt
\frac{17}{72} ...$$
The sequence of numbers $a_1,a_2,...$ which
appear in these rationals satisfies the
recurrence relation
$$a_{n+2}=4a_n+a_{n-1}$$
The two sequences
$\{p_{2k}/q_{2k}\}$ and
$\{p_{2k+1}/q_{2k+1}\}$ are
irrationally tuned, to $(\sqrt 5-1)/2$.
Compare Figures 1.1 and 1.2.
\newline
\newline
{\bf Cubical Limits:\/}
So far, I have only discussed the
situation when $\{B_k\}$ is always
the first block.
It is more natural to think of the
plaid model as taking place inside
the cube $[0,\omega]^3$.  What we
do is stack up the blocks of the
fundamental domain so that 
remotely adjacent blocks appear as
consecutive layers in the cube,
separated by $1/\omega$.  Once
this is done, the
four families of lines involved
in the plaid model include naturally
in $4$ families of planes.  One gets
the original lines by slicing the
planes by planes of the form
$z=k/\omega$ for $k=0,...,\omega-1$.

With this interpretation, the plaid
polygons become slices of {\it plaid surfaces\/}.
This point of view is familiar from
physics.  Instead of watching a curve
move through time in the plane, one
could interpret the moving curve as
slices of a surface in $2+1$ dimensional
spacetime.  

A more complete theory of rescaled
limits of the plaid model would involve
rescaling these cubes so that they
have unit side length.  This is
really equivalent to what we have said
above, but it organizes the various
limits so that the offsets vary in
a linear way with the slice.  In
short, the cube picture allows one
to consider all the possible rescaled
limits at once.  However, all these
considerations are for sequel papers.

\newpage


